NURBS-based finite element analysis of functionally graded plates: static bending, vibration, buckling and flutter

In this paper, a non-uniform rational B-spline based iso-geometric finite element method is used to study the static and dynamic characteristics of functionally graded material (FGM) plates. The material properties are assumed to be graded only in the thickness direction and the effective properties are computed either using the rule of mixtures or by Mori-Tanaka homogenization scheme. The plate kinematics is based on the first order shear deformation plate theory (FSDT). The shear correction factors are evaluated employing the energy equivalence principle and a simple modification to the shear correction factor is presented to alleviate shear locking. Static bending, mechanical and thermal buckling, linear free flexural vibration and supersonic flutter analysis of FGM plates are numerically studied. The accuracy of the present formulation is validated against available three-dimensional solutions. A detailed numerical study is carried out to examine the influence of the gradient index, the plate aspect ratio and the plate thickness on the global response of functionally graded material plates.

==> NurbsPlate/buckling.tex <==
\subsection{Buckling analysis}
In this section, we present the mechanical and thermal buckling behaviour of functionally graded skew plates. The FGM plate considered here consists of aluminum and alumina (see Table \ref{tab:matprop} for material properties).

%The Young's modulus, conductivity and the coefficient of thermal expansion for alumina is $E_c=$ 380 GPa, $K_c=$10.4 W/mK, $\alpha_c=$ 7.4 $\times$ 10$^{-6}$ 1/$^\circ$C, and for aluminum, $E_m=$ 70 GPa, $K_m=$ 204 W/mK, $\alpha_m=$ 23 $\times$ 10$^{-6}$ 1/$^\circ$C, respectively. Poisson's ratio is chosen as constant, $\nu=$ 0.3.

\subsubsection*{Mechanical Buckling}

%\begin{figure}[htpb]
%\centering
%\includegraphics[scale=1]{hyg.png}
%\caption{}
%\label{fig:mbuckLoad}
%\end{figure}

%\fref{fig:mbuckLoad} shows the loading directions considered in the present study. 
The critical buckling parameters are defined for uni- and bi- axial compressive loads as:

\begin{eqnarray}
\lambda_{\rm{cru}} = \frac{N_{\rm{xxcr}}^0 b^2}{\pi^2 D_c} \nonumber \\
\lambda_{\rm{crb}} = \frac{N_{\rm{yycr}}^0 b^2}{\pi^2 D_c} 
\label{eqn:mbuckparm}
\end{eqnarray}

where, $D_c=E_ch^3/(12(1-\nu^2))$. The critical buckling loads evaluated by varying the skew angle of the plate, volume fraction index and considering mechanical loads such as uni- and biaxial compressive loads are shown in Tables \ref{table:mbuckpah100}  - \ref{table:mbuckpah10} for two different thickness ratios. The efficacy of the present formulation is demonstrated by comparing our results with those in~\cite{ganapathiprakash2006}. It can be seen that increasing the gradient index decreases the critical buckling load. It is also observed that the decrease in the critical value is significant for the material gradient index $n \le 2$ and that further increase in $n$ yields less reduction in the critical value, irrespective of the skew angle. 

\begin{table}[htpb]
\renewcommand\arraystretch{1.5}
\caption{Critical buckling parameters for a thin simply supported FGM skew plate with $a/h=$ 100 and $a/b=$ 1.}
\centering
\begin{tabular}{ccccccccc}
\hline 
Skew angle & $\lambda_{cr}$ & \multicolumn{7}{c}{Gradient index, $n$} \\
\cline{3-9}
 &  & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & 2 & 5 & 10\\
\cline{3-6}
 &  & Ref.~\cite{ganapathiprakash2006} & Present & Ref.~\cite{ganapathiprakash2006} & Present \\
\hline
\multirow{2}{*}{0$^\circ$} & $\lambda_{\rm{cru}}$ & 4.0010 & 3.9998 & 1.7956 & 1.8034 & 1.5320 & 1.2606 & 1.0830 \\
& $\lambda_{\rm{crb}}$ & 2.0002 & 1.9999 & 0.8980 & 0.9017 & 0.7660 & 0.6303 & 0.5415 \\
\multirow{2}{*}{15$^\circ$} & $\lambda_{\rm{cru}}$ & 4.3946 & 4.3946 & 1.9716 & 1.9716 & 1.6752 & 1.3800 & 1.1868 \\
& $\lambda_{\rm{crb}}$ & 2.1154 & 2.1154 & 0.9517 & 0.9517 & 0.8086 & 0.6652 & 0.5716 \\
\multirow{2}{*}{30$^\circ$} & $\lambda_{\rm{cru}}$ & 5.8966 & 5.8966 & 2.6496 & 2.6496 & 2.2515 & 1.8607 & 1.6032 \\
& $\lambda_{\rm{crb}}$ & 2.5365 & 2.5365 & 1.1519 & 1.1519 & 0.9788 & 0.8044 & 0.6905 \\
\multirow{2}{*}{45$^\circ$} & $\lambda_{\rm{cru}}$ & 10.1031 & 10.1031 & 4.5445 & 4.5445 & 3.8625 & 3.2234 & 2.7964 \\
& $\lambda_{\rm{crb}}$ & 3.6399 & 3.6399 & 1.6863 & 1.6863 & 1.4330 & 1.1774 & 1.0103 \\
\hline
\end{tabular}
\label{table:mbuckpah100}
\end{table}

\begin{table}[htpb]
\renewcommand\arraystretch{1.5}
\caption{Critical buckling parameters for a thick simply supported FGM skew plate with $a/h=$ 10 and $a/b=$ 1.}
\centering
\begin{tabular}{ccccccccc}
\hline 
Skew angle & $\lambda_{cr}$ & \multicolumn{7}{c}{Gradient index, $n$} \\
\cline{3-9}
 &  & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} & 2 & 5 & 10\\
\cline{3-6}
 &  & Ref.~\cite{ganapathiprakash2006} & Present & Ref.~\cite{ganapathiprakash2006} & Present \\
\hline
\multirow{2}{*}{0$^\circ$} & $\lambda_{\rm{cru}}$ & 3.7374 & 3.7307 & 1.6892 & 1.6793 & 1.4198 & 1.1632 & 0.9999 \\
& $\lambda_{\rm{crb}}$ & 1.8686 & 1.8654 & 0.8449 & 0.8397 & 0.7099 & 0.5816 & 0.4999 \\
\multirow{2}{*}{15$^\circ$} & $\lambda_{\rm{cru}}$ & 4.0791 & 4.0791 & 1.8458 & 1.8458 & 1.5616 & 1.2810 & 1.1021 \\
& $\lambda_{\rm{crb}}$ & 1.9660 & 1.9660 & 0.8923 & 0.8923 & 0.7550 & 0.6184 & 0.5315 \\
\multirow{2}{*}{30$^\circ$} & $\lambda_{\rm{cru}}$ & 5.3571 & 5.3571 & 2.4298 & 2.4298 & 2.0533 & 1.6886 & 1.4565 \\
& $\lambda_{\rm{crb}}$ & 2.3226 & 2.3226 & 1.0659 & 1.0659 & 0.9011 & 0.7367 & 0.6326 \\
\multirow{2}{*}{45$^\circ$} & $\lambda_{\rm{cru}}$ & 8.5261 & 8.5261 & 3.8835 & 3.8835 & 3.2679 & 2.7046 & 2.3521 \\
& $\lambda_{\rm{crb}}$ & 3.1962 & 3.1962 & 1.5030 & 1.5030 & 1.2680 & 1.0335 & 0.8871 \\
\hline
\end{tabular}
\label{table:mbuckpah10}
\end{table}

%--------------------------------------------------------
%	Thermal buckling
%--------------------------------------------------------
\subsubsection*{Thermal Buckling}
The temperature rise of $T_m=$ 5$^\circ$C in the metal-rich surface of the plate is assumed in the present study. In addition to nonlinear temperature distribution across the plate thickness, the linear case is also considered in the present analysis by truncating the higher order terms in \Eref{eqn:heatconducres}. The plate is of uniform thickness and simply supported on all four edges. The critical buckling temperature difference $\Delta T_{cr}$ using two values of the aspect ratio $a/b=$ 1 and 2 with $a/h=10$ and for various skew angles is given in Table \ref{table:tbuckpah10}. It can been seen that the results from the present formulation are in good agreement with the results available in the literature. The decrease in the critical buckling load with the material gradient index $n$ is attributed to the stiffness degradation due to the increase in the metallic volume fraction. The thermal stability of the plate increases with the skew angle of the plate and the same behavior is observed for other values of gradient index $n$. It can also be seen that the nonlinear temperature variation through the thickness yields higher critical values compared to the linear distribution case.

\begin{table}[htpb]
\renewcommand\arraystretch{1.5}
\caption{Critical buckling temperature $\Delta T_{\rm{cr}}$ for a thin simply supported FGM skew plate with $a/h=$ 100 and $a/b=$ 1 under linear and nonlinear temperature rise through the thickness of the plate.}
\centering
\begin{tabular}{cclccccc}
\hline
$a/b$ & Skew angle & Temperature rise & \multicolumn{5}{c}{Gradient index, $n$} \\
\cline{4-8}
 &  &  & \multicolumn{2}{c}{0} & & &\\
\cline{4-5}
 &  &  & Ref.~\cite{ganapathiprakash2006a} & Present & 0.5 & 1 & 5 \\
\hline
\multirow{6}{*}{1} & \multirow{2}{*}{0$^\circ$} & Linear & 24.1951 & 24.1912 & 9.3787 & 5.5207 & 3.8987 \\
& & Nonlinear & 24.1951 & 24.1912 & 12.3629 & 7.6615 & 4.8740 \\
& \multirow{2}{*}{30$^\circ$} & Linear & 33.9558 & 33.9503 & 14.9115 & 9.7737 & 7.4681 \\
& & Nonlinear & 33.9558 & 33.9503 & 19.6600 & 13.558 & 9.3399 \\
& \multirow{2}{*}{60$^\circ$} & Linear & 123.0974 & 123.1172 & 65.4519 & 48.6271 & 40.0647 \\
& & Nonlinear & 123.0974 & 123.1172 & 86.2949 & 67.4989 & 50.1064 \\
\cline{3-8}
\multirow{3}{*}{2} & 0$^\circ$ & Nonlinear & 75.4278 & 75.4475 & 50.6564 & 38.6525 & 28.3067 \\
& 30$^\circ$ & Nonlinear & 100.9349 & 100.9512 & 69.7225 & 54.0838 & 39.9718 \\
& 60$^\circ$ & Nonlinear & 304.6912 & 304.6421 & 222.0921 & 177.4280 & 133.1456 \\
\hline
\end{tabular}
\label{table:tbuckpah10}
\end{table}

==> NurbsPlate/fgm.tex <==
\subsection{Functionally graded material}
A rectangular plate made of a mixture of ceramic and metal is considered with the coordinates $x,y$ along the in-plane directions and $z$ along the thickness direction (see \fref{fig:platefig}). The material on the top surface $(z=h/2)$ of the plate is ceramic rich and is graded to metal at the bottom surface of the plate $(z=-h/2)$ by a power law distribution. The effective properties of the FGM plate can be computed by using the rule of mixtures or by employing the Mori-Tanaka homogenization scheme.

Let $V_i (i=c,m)$ be the volume fraction of the phase material. The subscripts $c$ and $m$ refer to ceramic and metal phases, respectively. The volume fraction of ceramic and metal phases are related by $V_c + V_m = 1$ and $V_c$ is expressed as:

\begin{equation}
V_c(z) = \left( \frac{2z+h}{2h} \right)^n
\end{equation}

where $n$ is the volume fraction exponent $(n \geq 0)$, also known as the gradient index. The variation of the composition of ceramic and metal is linear for $n=$1, the value of $n=$ 0 represents a fully ceramic plate and any other value of $n$ yields a composite material with a smooth transition from ceramic to metal.

\subsubsection*{Rule of mixtures}
Based on the rule of mixtures, the effective property of a FGM is computed using the following expression:

\begin{equation}
P = P_c V_c + P_m V_m
\label{eqn:rulemix}
\end{equation}


\subsubsection*{Mori-Tanaka homogenization method}
Based on the Mori-Tanaka homogenization method, the effective Young's modulus and Poisson's ratio are computed from the effective bulk modulus $K$ and the effective shear modulus $G$ as~\cite{Sundararajan2005}

\begin{eqnarray}
\frac{K_{\rm eff}-K_m}{K_c-K_m} &=& \frac{V_c}{1 + V_m \frac{3(K_c-K_m)}{3K_m+4G_m}} \nonumber \\
\frac{G_{\rm eff}-G_m}{G_c-G_m} &=& \frac{V_c}{1 + V_m \frac{(G_c-G_m)}{(G_m+f_1)} }
\end{eqnarray}

where

\begin{equation}
f_1 = \frac{G_m (9K_m+8G_m)}{6(K_m+2G_m)}
\end{equation}

The effective Young's modulus $E_{\rm eff}$ and Poisson's ratio $\nu_{\rm eff}$ can be computed from the following relations:

\begin{eqnarray}
E_{\rm eff} = \frac{9 K_{\rm eff} G_{\rm eff}}{3K_{\rm eff} + G_{\rm eff}} \nonumber \\
\nu_{\rm eff} = \frac{3K_{\rm eff} - 2G_{\rm eff}}{2(3K_{\rm eff} + G_{\rm eff})}
\label{eqn:young}
\end{eqnarray}

The effective mass density $\rho$ is computed using the rule of mixtures. The effective heat conductivity $\kappa_{\rm eff}$ and the coefficient of thermal expansion $\alpha_{\rm eff}$ is given by:

\begin{eqnarray}
\frac{\kappa_{\rm eff} - \kappa_m}{\kappa_c - \kappa_m} = \frac{V_c}{1 + V_m \frac{(\kappa_c - \kappa_m)}{3\kappa_m}} \nonumber \\
\frac{\alpha_{\rm eff} - \alpha_m}{\alpha_c - \alpha_m} = \frac{ \left( \frac{1}{K_{\rm eff}} - \frac{1}{K_m} \right)}{\left(\frac{1}{K_c} - \frac{1}{K_m} \right)}
\label{eqn:thermalcondalpha}
\end{eqnarray}

\subsubsection*{Temperature distribution through the thickness}
The temperature variation is assumed to occur in the thickness direction only and the temperature field is considered to be constant in the $xy$-plane. In such a case, the temperature distribution along the thickness can be obtained by solving a steady state heat transfer problem:

\begin{equation}
-{d \over dz} \left[ \kappa(z) {dT \over dz} \right] = 0, \hspace{0.5cm} T = T_c ~\textup{at}~ z = h/2;~~ T = T_m ~\textup{at} ~z = -h/2
\label{eqn:heat}
\end{equation}

The solution of \Eref{eqn:heat} is obtained by means of a polynomial series~\cite{wu2004} as

\begin{equation}
T(z) = T_m + (T_c - T_m) \eta(z,h)
\label{eqn:tempsolu}
\end{equation}

where,

\begin{equation}
\begin{split}
\eta(z,h) = {1 \over C} \left[ \left( {2z + h \over 2h} \right) - {\kappa_{cm} \over (n+1)\kappa_m} \left({2z + h \over 2h} \right)^{n+1} + \right. \\ 
\left. {\kappa_{cm} ^2 \over (2n+1)\kappa_m ^2 } \left({2z + h \over 2h} \right)^{2n+1}
-{\kappa_{cm} ^3 \over (3n+1)\kappa_m ^3 } \left({2z + h \over 2h} \right)^{3n+1} \right. \\ + 
\left. {\kappa_{cm} ^4 \over (4n+1)\kappa_m^4 } \left({2z + h \over 2h} \right)^{4n+1} 
- {\kappa_{cm} ^5 \over (5n+1)\kappa_m ^5 } \left({2z + h \over 2h} \right)^{5n+1} \right] ;
\end{split}
\label{eqn:heatconducres}
\end{equation}

\begin{equation}
\begin{split}
C = 1 - {\kappa_{cm} \over (n+1)\kappa_m} + {\kappa_{cm} ^2 \over (2 n+1)\kappa_m ^2} 
- {\kappa_{cm} ^3 \over (3n+1)\kappa_m ^3} \\ + {\kappa_{cm} ^4 \over (4n+1)\kappa_m ^4}
- {\kappa_{cm} ^5\over (5n+1)\kappa_m ^5}
\end{split}
\end{equation}

==> NurbsPlate/flutter.tex <==
\subsection{Flutter analyses}
In this section, the present formulation is extended to analyse the flutter characteristics of functionally graded material plates. Both simply supported and clamped boundary conditions are considered in this study and the flow direction is assumed to be at right angles to the plate. Only square plate is considered and the results are presented only for $a/h=100$. It should be noted that the present formulation is not limited to this alone. In all cases, we present the non dimensionalized critical aerodynamic pressure, $\lambda_{cr}$ and critical frequency $\omega_{cr}$ as, unless specified otherwise:

\begin{eqnarray}
\Omega_{cr} = \omega_{cr} a^2 \sqrt{ \frac{\rho_c h}{D_c}} \nonumber \\
\lambda_{cr} = \lambda_{cr} \frac{a^3}{D_c}
\label{eqn:nondimfreq}
\end{eqnarray}

where $D_c = {E_c h^3 \over 12(1-\nu_c^2)}$ is the bending rigidity of the plate, $E_c, \nu_c$ are the Young's modulus and Poisson's ratio of the ceramic material and $\rho_c$ is the mass density. In order to be consistent with the existing literature, properties of the ceramic are used for normalization.


%\begin{eqnarray}
%u_o = w_o = \theta_y = 0 \hspace{1cm} ~\textup{on} ~ x=0,a \nonumber \\
%v_o = w_o = \theta_x = 0 \hspace{1cm} ~\textup{on} ~ y=0,b
%\end{eqnarray}

\begin{table}[htpb]
\renewcommand\arraystretch{1.5}
\caption{Comparison of critical aerodynamic pressure and coalescence frequency for an isotropic plate with various boundary conditions $(a/b=1, a/h=100, \nu=0.3, \theta^\prime = 0)$.}
\centering
\begin{tabular}{ccrr}
\hline 
Reference & Flutter bounds & \multicolumn{2}{c}{Boundary condition} \\
\cline{3-4}
1& 1 & Simply supported & Clamped \\
\hline
\multirow{2}{*}{Ref.~\cite{Prakash2006}} & $\lambda_{cr}$ & 511.11 & 852.34 \\
& $\omega_{cr}$ & 1840.29 & 4274.32 \\
\multirow{2}{*}{Present} & $\lambda_{cr}$ & 511.92 & 854.88 \\
& $\omega_{cr}$ & 1844.80 & 4305.30\\
\hline
\end{tabular}
\label{table:isoFlutComp}
\end{table}

Before proceeding with the detailed study, the formulation developed herein is validated against available results pertaining to the critical aerodynamic pressure and critical frequency for an isotropic plate with and without a crack. The computed critical aerodynamic pressure and the critical frequency for an isotropic square plate with various boundary conditions is given in  Table~\ref{table:isoFlutComp}. Next, the influence of boundary conditions on the flutter characteristics is studied. For this study, consider a square FGM plate made up of Aluminum-Alumina with $a/h=100$. \fref{fig:flutFGMRes} shows the influence of the boundary conditions on the critical aerodynamic pressure for various gradient index. It can be seen that the critical pressure is more for the clamped plate in comparison with that of the simply supported plate as expected. It is also seen that the aerodynamic pressure decreases with increase in the gradient index $n$. However the rate of decrease is high for low values of $n$. This can be attributed to the fact that the stiffness is high for the ceramic plate and minimum for the metallic plate and it degrades gradually with increase in the gradient index $n$. 

\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/flutResNurbs}
\caption{Effect of boundary conditions on the critical aerodynamic pressure $\lambda_{cr}$}
\label{fig:flutFGMRes}
\end{figure}

==> NurbsPlate/freevib.tex <==
\subsection{Free flexural vibrations}
In this section, the free flexural vibration characteristics of FGM plates are studied numerically. In all cases, we present the non-dimensionalized free flexural frequency defined as, unless otherwise stated:

\begin{equation}
\overline{\omega} = \omega h \sqrt{ \frac{\rho_c}{E_c}}
\end{equation}

where $\omega$ is the natural frequency, $\rho_c, E_c$ are the mass density and Young's modulus of the ceramic phase. Before proceeding with a detailed study on the effect of gradient index on the natural frequencies, the formulation developed herein is validated against available analytical/numerical solutions in the literature.

\subsubsection*{Square plates}
A  simply supported Al/Al$_2$O$_3$ FGM square plate with various length-to-thickness ratio is considered. The plate is modelled employing quadratic, cubic and quartic NURBS elements with meshes of 8, 14 and 20 control points per side. The results obtained from the isogeometric analysis for the first normalized frequency parameter $\overline{\omega}$ are presented in Tables \ref{tab:SSfgm1_freq1} and \ref{tab:SSfgm1_freq2} for different plate aspect ratios $(a/h=5,10,20)$ and compared with the results available in the literature~\cite{matsunaga2008,nguyen-xuantran2011,zhaolee2009,hashemifadaee2011}. The first normalized frequency $(= \overline{\omega}/\omega_{analytical})$ is shown in \frefs{fig:normfreqah5} - \fref{fig:normfreqah20} for various $a/h$ ratios $(a/h=5,10,20)$. The results of IGA shown in these figures are computed using quadratic NURBS elements with 14 control points per side. It is seen that the results from IGA are superior to compared to other methods, irrespective of the material gradient index.

% of the edge based smoothed stabilized discrete shear gap element (ES-DSG3)~\cite{nguyen-xuantran2011}, MITC4 and DSG3~\cite{nguyen-xuantran2011}, element free $kp-$Ritz method~\cite{zhaolee2009}, higher order shear deformation theory~\cite{matsunaga2008} and an exact analytical approach~\cite{hashemifadaee2011}. The first frequency normalized to the analytical solution~\cite{hashemifadaee2011} versus various volume fraction exponents is plotted in \frefs{fig:normfreqah5} - \ref{fig:normfreqah20} for different $a/h$ ratios. The results of IGA presented in these figures obtained using quadratic NURBS elements with 14 control points per side. It is seen that for $a/h=$ 5, the best results are gained using IGA and MITC4 methods. For $a/h=$ 10, IGA gains the best results comparing with other methods. The same behaviour can be found for $a/h=$ 20. 

% normalized frequency for a/h=5, a/h=10/ a/h=20
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/fig6}
\caption{The normalized first frequency $\omega^\ast = \omega/\omega_{\rm{ref}}$ versus volume fraction exponents for SSSS Al/Al$_2$O$_3$ FGM plate with $a/h=$ 5. The frequency is normalized with the analytical solution.}
\label{fig:normfreqah5}
\end{figure}

\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/fig7}
\caption{The normalized first frequency $\omega^\ast = \omega/\omega_{\rm{ref}}$ versus volume fraction exponents for SSSS Al/Al$_2$O$_3$ FGM plate with $a/h=$ 10. The frequency is normalized with the analytical solution.}
\label{fig:normfreqah10}
\end{figure}

\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/fig8}
\caption{The normalized first frequency $\omega^\ast = \omega/\omega_{\rm{ref}}$ versus volume fraction exponents for SSSS Al/Al$_2$O$_3$ FGM plate with $a/h=$ 20. The frequency is normalized with the analytical solution.}
\label{fig:normfreqah20}
\end{figure}

% frequency for various boundary conditions...and different modes
\begin{figure}[htpb]
\centering
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig9a}}
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig9b}}
\caption{The non-dimensional frequency $\overline{\omega} = \frac{\omega a^2}{h} \sqrt{ \frac{\rho_c}{E_o} }$ versus various volume fraction exponent of Al/ZrO$_2$ FGM plate with different boundary conditions: (a) Mode 1 and (b) Mode 2.}
\label{fig:first2modes}
\end{figure}

\begin{figure}[htpb]
\centering
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig9c}}
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig9d}}
\caption{The non-dimensional frequency $\overline{\omega} = \frac{\omega a^2}{h} \sqrt{ \frac{\rho_c}{E_o} }$ versus various volume fraction exponent of Al/ZrO$_2$ FGM plate with different boundary conditions: (a) Mode 3 and (b) Mode 4.}
\label{fig:second2modes}
\end{figure}

\frefs{fig:first2modes} - (\ref{fig:second2modes}) shows the first four non-dimensionalized frequencies for a Al/ZrO$_2$ FGM plate with $a/h=$ 10 with various boundary conditions (CCCC, SSSS and CFFF). It can be seen that very good agreement is obtained with the results available in the literature. For CFFF boundary conditions, the difference between the IGA and the element free $kp-$Ritz is ranged from 0.3\% to 2.1\%, while it is about 2.2 - 3.3\% and 1.6 - 2.5\% for CCCC and SSSS boundary conditions, respectively. Note that all the present results agree very well with those given in~\cite{nguyen-xuantran2012,nguyen-xuantran2011}.

% normalized frequencies for fully SSSS Al/Al2O3 square plate
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{The first normalized frequency parameter $\overline{\omega} = \omega h \sqrt{\frac{\rho_c}{E_c}}$ for fully simply supported Al/Al$_2$O$_3$ FGM square plate for $a/h=$ 5.}
\begin{tabular}{llrrrrr}
\hline
Method & Control points & \multicolumn{5}{c}{gradient index $n$} \\
\cline{3-7}
 &  & 0 & 0.5 & 1 & 4 & 10\\
\hline
\multirow{3}{*}{IGA-Quadratic} & 8 & 0.21128 & 0.18051 & 0.16309 & 0.13962 & 0.13231 \\
& 14 & 0.21121 & 0.18045 & 0.16303 & 0.13957 & 0.13227 \\
& 20 & 0.21121 & 0.18044 & 0.16303 & 0.13957 & 0.13227 \\
\cline{3-7}
\multirow{3}{*}{IGA-Cubic} & 8 & 0.21121 & 0.18044 & 0.16303 & 0.13957 & 0.13227 \\
& 14 & 0.21121 & 0.18044 & 0.16303 & 0.13957 & 0.13227 \\
& 20 & 0.21121 & 0.18044 & 0.16303 & 0.13957 & 0.13227 \\
\cline{3-7}
\multirow{3}{*}{IGA-Quartic} & 8 & 0.21121 & 0.18044 & 0.16303 & 0.13957 & 0.13227 \\
& 14 & 0.21121 & 0.18044 & 0.16303 & 0.13957 & 0.13227 \\
& 20 & 0.21121 & 0.18044 & 0.16303 & 0.13957 & 0.13227 \\
\cline{3-7}
ES-DSG3 (20$\times$20)~\cite{nguyen-xuantran2011} & & 0.21218 & 0.18114 & 0.16351 & 0.13992 & 0.13272 \\
DSG3 (16$\times$16)~\cite{nguyen-xuantran2011} & & 0.21335 & 0.18216 & 0.16444 & 0.14069 & 0.13343 \\
MITC4 (16$\times$16)~\cite{nguyen-xuantran2011} & & 0.21182 & 0.18082 & 0.16323 & 0.13968 & 0.13251 \\
HSDT~\cite{matsunaga2008} & & 0.21210 & 0.18190 & 0.16400 & 0.13830 & 0.13060 \\
$kp-$Ritz~\cite{zhaolee2009} & & 0.20550 & 0.17570 & 0.15870 & 0.13560 & 0.12840 \\
Ref.~\cite{hashemifadaee2011} & & 0.21120 & 0.18050 & 0.16310 & 0.13970 & 0.13240 \\
\hline
\end{tabular}%
\label{tab:SSfgm1_freq1}%
\end{table}%

\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{The first normalized frequency parameter $\overline{\omega} = \omega h \sqrt{\frac{\rho_c}{E_c}}$ for fully simply supported Al/Al$_2$O$_3$ FGM square plate for $a/h=$ 10, 20.}
\begin{tabular}{clrrrrr}
\hline
$a/h$ & Method & \multicolumn{5}{c}{gradient index $n$} \\
\cline{4-7}
 &  & 0 & 0.5 & 1 & 4 & 10\\
\hline
\multirow{9}{*}{10} & IGA-Quadratic (20 points)  & 0.05769 & 0.04899 & 0.4418 & 0.03821 & 0.03655 \\
& IGA-Cubic (20 points) & 0.05769 & 0.04898 & 0.04417 & 0.03821 & 0.03655 \\
& IGA-Quartic (20 points) & 0.05769 & 0.04898 & 0.04417 & 0.03821 & 0.03655 \\
& ES-DSG3 (20$\times$20)~\cite{nguyen-xuantran2011}  & 0.05800 & 0.04924 & 0.04439 & 0.03839 & 0.03973 \\
& DSG3 (16$\times$16)~\cite{nguyen-xuantran2011}  & 0.05834 & 0.04954 & 0.04467 & 0.03861 & 0.03693 \\
& MITC4 (16$\times$16)~\cite{nguyen-xuantran2011}  & 0.05787 & 0.049132 & 0.04429 & 0.03830 & 0.03665 \\
& HSDT~\cite{matsunaga2008}  & 0.05777 & 0.04917 & 0.04426 & 0.03811 & 0.03642 \\
& $kp-$Ritz~\cite{zhaolee2009}  & 0.05673 & 0.04818 & 0.04346 & 0.3757 & 0.03591 \\
& Ref.~\cite{hashemifadaee2011}  & 0.05770 & 0.04900 & 0.04420 & 0.03820 & 0.03660 \\
\cline{2-7}
\multirow{9}{*}{20} & IGA-Quadratic (20 points) & 0.01480 & 0.01254 & 0.01130 & 0.00981 & 0.00944 \\
& IGA-Cubic (20 points) & 0.01480 & 0.01254 & 0.01130 & 0.00981 & 0.00944 \\
& IGA-Quartic (20 points) & 0.01480 & 0.01254 & 0.01130 & 0.00981 & 0.00944 \\
& ES-DSG3 (20$\times$20)~\cite{nguyen-xuantran2011}  & 0.01488 & 0.01261 & 0.01137 & 0.00986 & 0.00946 \\
& DSG3 (16$\times$16)~\cite{nguyen-xuantran2011} &  0.01498 & 0.012704 & 0.01145 & 0.00993 & 0.00952 \\
& MITC4 (16$\times$16)~\cite{nguyen-xuantran2011}  & 0.01485 & 0.01258 & 0.01134 & 0.00984 & 0.00944 \\
& $kp-$Ritz~\cite{zhaolee2009} &  0.01464 & 0.01241 & 0.01118 & 0.00970 & 0.00931 \\
& Ref.~\cite{hashemifadaee2011} & 0.01480 & 0.01250 & 0.01130 & 0.00980 & 0.00940 \\
\hline
\end{tabular}%
\label{tab:SSfgm1_freq2}%
\end{table}%

%-------------------- Skew plates
\subsubsection*{Skew plate}
Next, the effects of the skewness of the plate on the free flexural vibration of the FGM plate is studied. A Al/ZrO$_2$-2 skew FGM plate with length-to-thickness ratio $a/h=$ 10 and various skew angles are considered in this example. The skew plate is modelled using quadratic NURBS elements with 17 $\times$ 17 control points. The first two non-dimensionalized frequencies are shown in \frefs{fig:skewFreq_ah10_SS} - (\ref{fig:skewFreq1_ah10_CC}) for SSSS and CCCC boundary conditions, respectively. For comparison, the results from the element free $kp-$Ritz~\cite{zhaolee2009} are also plotted. From the figures, it is seen that the IGA gives higher frequencies than the element free $kp-$Ritz method. It is also observed that by increasing the gradient index or decreasing the skew angle, the frequency decreases. In both cases, the decrease in the natural frequency can be attributed to the stiffness degradation. In the case of gradient index, the stiffness degradation is due to increased metallic volume fraction, while the geometry of the plate is a contributing factor in decreasing the frequency when the skew angle decreases. The first eight mode shapes of fully clamped Al/ZrO$_2$-2 skew plate with skew angle $\psi=$ 45$^\circ$ and gradient index $n=$ 0.5 is plotted in \fref{fig:skewFreq_ah10_CC}. 

% non dimensional frequency for SSSS with a/h=10
\begin{figure}[htpb]
\centering
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig16-1}}
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig16-2}}
\caption{The non-dimensional frequency $\overline{\omega} = \omega a^2 \sqrt{\rho_c/E_c}$ for a simply supported Al/ZrO$_2$-2 skew plate versus various skew angles for different values of gradient index with $a/h=$ 10.}
\label{fig:skewFreq_ah10_SS}
\end{figure}

% non dimensional frequency for CCCC with a/h=10
\begin{figure}[htpb]
\centering
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig17-1}}
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig17-2}}
\caption{The non-dimensional frequency $\overline{\omega} = \omega a^2 \sqrt{\rho_c/E_c}$ for a clamped Al/ZrO$_2$-2 skew plate versus various skew angles for different values of gradient index with $a/h=$ 10.}
\label{fig:skewFreq1_ah10_CC}
\end{figure}

% non dimensional frequency for CCCC with a/h=10
\begin{figure}[htpb]
\centering
\subfigure[mode 1]{\includegraphics[scale=0.25]{./Figures/fig18-1}}
\subfigure[mode 2]{\includegraphics[scale=0.25]{./Figures/fig18-2}}
\subfigure[mode 3]{\includegraphics[scale=0.25]{./Figures/fig18-3}}
\subfigure[mode 4]{\includegraphics[scale=0.25]{./Figures/fig18-4}}
\subfigure[mode 5]{\includegraphics[scale=0.25]{./Figures/fig18-5}}
\subfigure[mode 6]{\includegraphics[scale=0.25]{./Figures/fig18-6}}
\subfigure[mode 7]{\includegraphics[scale=0.25]{./Figures/fig18-7}}
\subfigure[mode 8]{\includegraphics[scale=0.25]{./Figures/fig18-8}}
\caption{First eight mode shapes for a clamped Al/Zro$_2$ skew plate with $a/h=$ 10, gradient index $n=$ 0.5 and $\psi=$ 45$^\circ$.}
\label{fig:skewFreq_ah10_CC}
\end{figure}

==> NurbsPlate/plate.pstex_t.tex <==
\begin{picture}(0,0)%
\includegraphics{plate.pstex}%
\end{picture}%
\setlength{\unitlength}{2279sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(7002,4165)(2689,-5264)
\put(4501,-5191){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}$a$}}}}
\put(8371,-3481){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}$b$}}}}
\put(9676,-1861){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}$h$}}}}
\end{picture}%


==> NurbsPlate/plateTheory.tex <==
\subsection{Reissner-Mindlin Plates}
The displacements $u,v,w$ at a point $(x,y,z)$ in the plate (see \fref{fig:platefig}) from the medium surface are expressed as functions of the mid-plane displacements $u_o,v_o,w_o$ and independent rotations $\theta_x,\theta_y$ of the normal in $yz$ and $xz$ planes, respectively, as:

\begin{eqnarray}
u(x,y,z,t) &=& u_o(x,y,t) + z \theta_x(x,y,t) \nonumber \\
v(x,y,z,t) &=& v_o(x,y,t) + z \theta_y(x,y,t) \nonumber \\
w(x,y,z,t) &=& w_o(x,y,t) 
\label{eqn:displacements}
\end{eqnarray}

where $t$ is the time. 

\begin{figure}[htpb]
\centering
\subfigure[]{\input{plate.pstex_t}}
\subfigure[]{\input{skew.pstex_t}}
\caption{(a) coordinate system of a rectangular FGM plate, (b) Coordinate system of a skew plate}
\label{fig:platefig}
\end{figure}

The strains in terms of mid-plane deformation can be written as:

\begin{equation}
\bveps  = \left\{ \begin{array}{c} \bveps_p \\ 0 \end{array} \right \}  + \left\{ \begin{array}{c} z \bveps_b \\ \bveps_s \end{array} \right\} 
\label{eqn:strain1}
\end{equation}

The midplane strains $\bveps_p$, bending strain $\bveps_b$, shear strain $\varepsilon_s$ in \Eref{eqn:strain1} are written as:

\begin{eqnarray}
\renewcommand{\arraystretch}{1.2}
\bveps_p = \left\{ \begin{array}{c} u_{o,x} \\ v_{o,y} \\ u_{o,y}+v_{o,x} \end{array} \right\}, \hspace{1cm}
\renewcommand{\arraystretch}{1.2}
\bveps_b = \left\{ \begin{array}{c} \theta_{x,x} \\ \theta_{y,y} \\ \theta_{x,y}+\theta_{y,x} \end{array} \right\}, \nonumber \\
\renewcommand{\arraystretch}{1.2}
\bveps_s = \left\{ \begin{array}{c} \theta _x + w_{o,x} \\ \theta _y + w_{o,y} \end{array} \right\}. \hspace{1cm}
\renewcommand{\arraystretch}{1.2}
\end{eqnarray}

where the subscript `comma' represents the partial derivative with respect to the spatial coordinate succeeding it. The membrane stress resultants $\bn$ and the bending stress resultants $\bfm$ can be related to the membrane strains, $\bveps_p$ and bending strains $\bveps_b$ through the following constitutive relations:

\begin{eqnarray}
\bn &=& \left\{ \begin{array}{c} N_{xx} \\ N_{yy} \\ N_{xy} \end{array} \right\} = \mathbf{A} \bveps_p + \BB \bveps_b \nonumber \\
\bfm &=& \left\{ \begin{array}{c} M_{xx} \\ M_{yy} \\ M_{xy} \end{array} \right\} = \BB \bveps_p + \DD \bveps_b 
\end{eqnarray}

where the matrices $\mathbf{A} = A_{ij}, \BB= B_{ij}$ and $\DD = D_{ij}; (i,j=1,2,6)$ are the extensional, bending-extensional coupling and bending stiffness coefficients and are defined as:

\begin{equation}
\left\{ A_{ij}, ~B_{ij}, ~ D_{ij} \right\} = \int_{-h/2}^{h/2} \overline{Q}_{ij} \left\{1,~z,~z^2 \right\}~dz
\end{equation}

Similarly, the transverse shear force $Q = \{Q_{xz},Q_{yz}\}$ is related to the transverse shear strains $\varepsilon_s$ through the following equation:

\begin{equation}
Q_{ij} = E_{ij} \varepsilon_s
\end{equation}

where $E_{ij} = \int_{-h/2}^{h/2} \overline{Q} \upsilon_i \upsilon_j~dz;~ (i,j=4,5)$ is the transverse shear stiffness coefficient, $\upsilon_i, \upsilon_j$ is the transverse shear coefficient for non-uniform shear strain distribution through the plate thickness. The stiffness coefficients $\overline{Q}_{ij}$ are defined as:

\begin{eqnarray}
\overline{Q}_{11} = \overline{Q}_{22} = {E(z) \over 1-\nu^2}; \hspace{1cm} \overline{Q}_{12} = {\nu E(z) \over 1-\nu^2}; \hspace{1cm} \overline{Q}_{16} = \overline{Q}_{26} = 0 \nonumber \\
\overline{Q}_{44} = \overline{Q}_{55} = \overline{Q}_{66} = {E(z) \over 2(1+\nu) }
\end{eqnarray}

where the modulus of elasticity $E(z)$ and Poisson's ratio $\nu$ are given by \Eref{eqn:young}. The thermal stress resultant $\bn^{\rm th}$ and the moment resultant $\bfm^{\rm th}$ are:

\begin{eqnarray}
\bn^{\rm th}&=& \left\{ \begin{array}{c} N^{\rm th}_{xx} \\ N^{\rm th}_{yy} \\ N^{\rm th}_{xy} \end{array} \right\} = \int\limits_{-h/2}^{h/2} \overline{Q}_{ij} \alpha(z,T) \left\{ \begin{array}{c} 1 \\ 1 \\ 0 \end{array} \right\} \Delta T(z)~ \rmd z \nonumber \\
\bfm^{\rm th} &=& \left\{ \begin{array}{c} M^{\rm th}_{xx} \\ M^{\rm th}_{yy} \\ M^{\rm th}_{xy} \end{array} \right\} = \int\limits_{-h/2}^{h/2} \overline{Q}_{ij} \alpha(z,T) \left\{ \begin{array}{c} 1 \\ 1 \\ 0 \end{array} \right\} \Delta T(z)~ z ~\rmd z \nonumber \\ 
\end{eqnarray}

where the thermal coefficient of expansion $\alpha(z,T)$ is given by \Eref{eqn:thermalcondalpha} and $\Delta T(z) = T(z)-T_o$ is the temperature rise from the reference temperature and $T_o$ is the temperature at which there are no thermal strains. The strain energy function $U$ is given by:

\begin{equation}
\begin{split}
U(\boldsymbol{\delta}) = {1 \over 2} \int_{\Omega} \left\{ \bveps_p^{\textup{T}} \mathbf{A} \bveps_p + \bveps_p^{\textup{T}} \mathbf{B} \bveps_b + 
\bveps_b^{\textup{T}} \mathbf{B} \bveps_p + \bveps_b^{\textup{T}} \mathbf{D} \bveps_b +  \bveps_s^{\textup{T}} \mathbf{E} \bveps_s \right\}~ \mathrm{d} \Omega
\end{split}
\label{eqn:potential}
\end{equation}

where $\boldsymbol{\delta} = \{u,v,w,\theta_x,\theta_y\}$ is the vector of the degree of freedom associated to the displacement field in a finite element discretization. Following the procedure given in~\cite{Rajasekaran1973}, the strain energy function $U$ given in~\Eref{eqn:potential} can be rewritten as:

\begin{equation}
U(\boldsymbol{\delta}) = {1 \over 2}  \boldsymbol{\delta}^{\textup{T}} \mathbf{K}  \boldsymbol{\delta}
\label{eqn:poten}
\end{equation}

where $\mathbf{K}$ is the linear stiffness matrix. The kinetic energy of the plate is given by:

\begin{equation}
T(\boldsymbol{\delta}) = {1 \over 2} \int_{\Omega} \left\{p (\dot{u}_o^2 + \dot{v}_o^2 + \dot{w}_o^2) + I(\dot{\theta}_x^2 + \dot{\theta}_y^2) \right\}~\mathrm{d} \Omega
\label{eqn:kinetic}
\end{equation}

where $p = \int_{-h/2}^{h/2} \rho(z)~dz, ~ I = \int_{-h/2}^{h/2} z^2 \rho(z)~dz$ and $\rho(z)$ is the mass density that varies through the thickness of the plate. When the plate is subjected to a temperature field, this in turn results in in-plane stress resultants, $\bn^{\rm th}$. The external work due to the in-plane stress resultants developed in the plate under a thermal load is given by:

\begin{equation}
\begin{split}
V(\boldsymbol{\delta}) = \int\limits_\Omega \left\{ \frac{1}{2} \left[ N_{xx}^{\rm th} w_{,x}^2 + N_{yy}^{\rm th} w_{,y}^2 + 2 N_{xy}^{\rm th}w_{,x}w_{,y}\right] + \right. \\ \left.
\frac{h^2}{24} \left[ N_{xx}^{\rm th} \left( \theta_{x,x}^2 + \theta_{y,x}^2 \right) + N_{yy}^2 \left( \theta_{x,y}^2 + \theta_{y,y}^2 \right) + 2 N_{xy}^{\rm th} \left( \theta_{x,x}\theta_{x,y} + \theta_{y,x}\theta_{y,y} \right) \right] \right\}~ d\Omega
\end{split}
\end{equation}

The governing equations of motion are obtained by writing the Lagrange equations of motion given by:

\begin{equation}
\frac{d}{dt} \left[ \frac{\partial(T-U)}{\partial \dot{\boldsymbol{\delta}}_i} \right] - \left[ \frac{\partial(T-U)}{\partial \boldsymbol{\delta}_i} \right] = 0, \hspace{0.5cm} i=1,2,\cdots,n
\end{equation}

The governing equations obtained using the minimization of total potential energy are solved using Galerkin finite element method. The finite element equations thus derived are:

{\bf Static bending}: 
\begin{equation}
\left( \KK + \KK_G \right) \boldsymbol{\delta} = \mathbf{F}
\label{eqn:staticgovern}
\end{equation}

{\bf Free vibration}: 
\begin{equation}
\bfm \ddot{\boldsymbol{\delta}} + \left( \KK + \KK_G \right) \boldsymbol{\delta} = \mathbf{0}
\label{eqn:freevibgovern}
\end{equation}


{\bf Buckling analysis}:

\paragraph*{Mechanical Buckling}
\begin{equation}
\left( \KK + \lambda \KK_G \right) \boldsymbol{\delta} = \mathbf{0}
\end{equation}


\paragraph*{Thermal Buckling}
\begin{equation}
\left( \KK + \Delta T \KK_G \right) \boldsymbol{\delta} = \mathbf{0}
\end{equation}

where $\boldsymbol{\delta}$ is the vector of degree of freedom associated to the displacement field in a finite element discretization, $\Delta T(=T_c - T_m)$ is the critical temperature difference, $\lambda$ is the critical buckling load and $\KK$, $\KK_G$ are the linear stiffness and geometric stiffness matrices, respectively. The critical temperature difference is computed using a standard eigenvalue algorithm. \\


{\bf Flutter analysis}: 
% for aerodynamic loading....
The work done by the applied non-conservative loads is:
\begin{equation}
W(\boldsymbol{\delta}) = \int_{\Omega} \Delta p w ~\rmd \Omega
\label{eqn:aerowork}
\end{equation}

where $\Delta p$ is the aerodynamic pressure. The aerodynamic pressure based on first-order, high Mach number approximation to linear potential flow is given by:

\begin{equation}
\Delta p = \frac{\rho_a U_a^2}{\sqrt{M_\infty^2 - 1}} \left[ \frac{\partial w}{\partial x} \cos \theta^\prime + \frac{\partial w}{\partial y} \sin \theta^\prime + \left( \frac{1}{U_a} \right) \frac{M_\infty^2 - 2}{M_\infty^2 - 1} \frac{\partial w}{\partial t} \right]
\label{eqn:aeropressure}
\end{equation}

where $\rho_a, U_a, M_\infty$ and $\theta^\prime$ are the free stream air density, velocity of air, Mach number and flow angle, respectively. The static aerodynamic approximation for Mach numbers between $\sqrt{2}$ and $2$ is~\citep{Birman1990}:

\begin{equation}
\Delta p = \frac{\rho_a U_a^2}{\sqrt{M_\infty^2 - 1}} \left[ \frac{\partial w}{\partial x} \cos \theta^\prime + \frac{\partial w}{\partial y} \sin \theta^\prime  \right]
\label{eqn:aeropressurestat}
\end{equation}

Substituting \Eref{eqn:poten} - (\ref{eqn:aerowork}) in Lagrange's equations of motion, the following governing equation is obtained:

\begin{equation}
\bfm \ddot{\boldsymbol{\delta}} + (\KK + \lambda \overline{\mathbf{A}}) \boldsymbol{\delta} = \mathbf{0}
\label{eqn:govereqn}
\end{equation}

After substituting the characteristic of the time function~\cite{Ganapathi1996} $\ddot{\boldsymbol{\delta}} = -\omega^2 \boldsymbol{\delta}$, the following algebraic equation is obtained:

\begin{equation}
\left[ \left( \KK + \lambda \overline{\mathbf{A}}\right) - \omega^2 \bfm\right] \boldsymbol{\delta} = \mathbf{0}
\label{eqn:finaldiscre}
\end{equation}

where $\KK$ is the stiffness matrix, $\bfm$ is the consistent mass matrix, $\lambda = \frac{\rho_a U_a^2}{\sqrt{M_\infty^2 - 1}}$, $\overline{\mathbf{A}}$ is the aerodynamic force matrix and $\omega$ is the natural frequency. When $\lambda = $0, the eigenvalue of $\omega$ is real and positive, since the stiffness matrix and mass matrix are symmetric and positive definite. However, the aerodynamic matrix $\overline{\mathbf{A}}$ is unsymmetric and hence complex eigenvalues $\omega$ are expected for $\lambda >$ 0. As $\lambda$ increases monotonically from zero, two of these eigenvalues will approach each other and become complex conjugates. In this study, $\lambda_{cr}$ is considered to be the value of $\lambda$ at which the first coalescence occurs.


%--------------------------- not used
%where $\omega$ is the natural frequency. In the present study, while performing the integration, terms having thickness co-ordinate $z$ are integrated with higher order Gaussian quadrature, because the material properties vary continuously through the thickness. The terms containing $x$ and $y$ are evaluated using full integration with 3 $\times$ 3 Gauss integration rule. The frequencies are obtained from \Eref{eqn:finaldiscre} using the generalized eigenvalue algorithm. \\


==> NurbsPlate/skew.pstex_t.tex <==
\begin{picture}(0,0)%
\includegraphics{skew.pstex}%
\end{picture}%
\setlength{\unitlength}{2279sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(6804,3835)(2659,-5039)
\put(2746,-4156){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}$\psi$}}}}
\put(2746,-2671){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}$y$}}}}
\put(5491,-1411){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}$y^\prime$}}}}
\put(7606,-4471){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}$x,x^\prime$}}}}
\put(4636,-4966){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}$a$}}}}
\put(8371,-3301){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}$b$}}}}
\end{picture}%


==> NurbsPlate/static.tex <==
\subsection{Static Bending}

%\subsubsection*{Convergence study of FGM plates under mechanical loads}
Let us consider a Al/ZrO$_2$ FGM square plate with length-to-thickness $a/h=$ 5, subjected to a uniform load with fully simply supported (SSSS) and fully clamped (CCCC) boundary conditions. Four different values for the gradient index $(n=0,0.5,1,2)$ are considered in this study. The plate is modelled with 4, 8, 16, 24 and 32 control points per side. Tables \ref{tab:SSfgm1_static} and \ref{tab:CCfgm1_static} summarize the IGA results with quadratic, cubic and quartic NURBS elements for SSSS and CCCC boundary conditions. It can be seen that for all polynomial orders, the convergence of the results is quite fast. For cubic and quartic NURBS elements, the convergence is almost achieved with 16 control points per side. Table \ref{tab:ssss-cccc-valid} compares the results from the present formulation with other approaches available in the literature~\cite{gilhooleybatra2007,leezhao2009,nguyen-xuantran2012} and a very good agreement can be observed.

%For the comparison purpose, the IGA solutions using the mesh of 13 $\times$ 13 control points with different order of NURBS are considered and compared with the results of MLPG~\cite{gilhooleybatra2007}, $kp-$Ritz~\cite{leezhao2009}, MITC4~\cite{nguyen-xuantran2012}, ES-DSG3~\cite{nguyen-xuantran2012} and NS-DSG3~\cite{nguyen-xuantran2012}. From Table \ref{tab:ssss-cccc-valid}, a very good agreement between the IGA results and those obtained by other approaches can be found.

% normalized center deflection of Simply Supported Al/ZrO2-1 FGM plate
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{The normalized center deflection for fully simply supported Al/ZrO$_2$-1 FGM square plate with $a/h=$ 5, subjected to a uniformly distributed load $p$ using IGA. $^\ast$At least 5 control points per side are needed for 1 quartic NURBS element.}
\begin{tabular}{cccccc}
\hline
Method & Number of & \multicolumn{4}{c}{gradient index, $n$} \\
\cline{3-6}
& Control Points & 0 & 0.5 & 1 & 2 \\
\hline
\multirow{5}{*}{Quadratic} & 4 & 0.162098 & 0.218914 & 0.256018 & 0.293806 \\
& 8 & 0.171617 & 0.232392 & 0.271879 & 0.311459 \\
& 16 & 0.171649 & 0.232439 & 0.271935 & 0.311520 \\
& 24 & 0.171651 & 0.232441 & 0.271938 & 0.311523 \\
& 32 & 0.171651 & 0.232442 & 0.271938 & 0.311523 \\
\cline{2-6}
\multirow{5}{*}{Cubic} & 4 & 0.163329 & 0.220598 & 0.257991 & 0.296053 \\
& 8 & 0.171658 & 0.232452 & 0.271950 & 0.311536 \\
& 16 & 0.171651 & 0.232441 & 0.271938 & 0.311522 \\
& 24 & 0.171651 & 0.232442 & 0.271938 & 0.311523 \\
& 32 & 0.171651 & 0.232442 & 0.271938 & 0.311523 \\
\cline{2-6}
\multirow{5}{*}{Quartic} & 5$^\ast$ & 0.172910 & 0.234167 & 0.273959 & 0.313821 \\
& 8 & 0.171690 & 0.232495 & 0.272000 & 0.311594 \\
& 16 & 0.171651 & 0.232442 & 0.271938 & 0.311523 \\
& 24 & 0.171651 & 0.232442 & 0.271938 & 0.311523 \\
& 32 & 0.171651 & 0.232442 & 0.271938 & 0.311523 \\
\hline
\end{tabular}%
\label{tab:SSfgm1_static}%
\end{table}%

% normalized center deflection of fully clamped Al/ZrO2-1 FGM plate
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{The normalized center deflection for fully clamped Al/ZrO$_2$-1 FGM square plate with $a/h=$ 5, subjected to a uniformly distributed load $p$ using IGA. $^\ast$At least 5 control points per side are needed for 1 quartic NURBS element.}
\begin{tabular}{cccccc}
\hline
Method & Number of & \multicolumn{4}{c}{gradient index, $n$} \\
\cline{3-6}
& Control Points & 0 & 0.5 & 1 & 2 \\
\hline
\multirow{5}{*}{Quadratic} & 4 & 0.052510 & 0.06818 & 0.079306 & 0.093421 \\
& 8 & 0.075831 & 0.101036 & 0.117946 & 0.136557 \\
& 16 & 0.076017 & 0.101305 & 0.118264 & 0.136905 \\
& 24 & 0.076024 & 0.101315 & 0.118276 & 0.136918 \\
& 32 & 0.076025 & 0.101316 & 0.118278 & 0.136920 \\
\cline{2-6}
\multirow{5}{*}{Cubic} & 4 & 0.056337 & 0.07342 & 0.085447 & 0.100403 \\
& 8 & 0.076031 & 0.101324 & 0.118287 & 0.136931 \\
& 16 & 0.076025 & 0.101316 & 0.118277 & 0.136921 \\
& 24 & 0.076025 & 0.101317 & 0.118278 & 0.136921 \\
& 32 & 0.076026 & 0.101317 & 0.118279 & 0.136921 \\
\cline{2-6}
\multirow{5}{*}{Quartic} & 5$^\ast$ & 0.077690 & 0.103620 & 0.120980 & 0.139973 \\
& 8 & 0.076092 & 0.101409 & 0.118387 & 0.137043 \\
& 16 & 0.076026 & 0.101317 & 0.118279 & 0.136921 \\
& 24 & 0.076026 & 0.101317 & 0.118279 & 0.136921 \\
& 32 & 0.076026 & 0.101317 & 0.118279 & 0.136921 \\
\hline
\end{tabular}%
\label{tab:CCfgm1_static}%
\end{table}%

% validation with previously published results
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{The normalized center deflection for fully clamped Al/ZrO$_2$-1 FGM square plate with $a/h=$ 5, subjected to a uniformly distributed load $p$ using 13 $\times$13 control points for various boundary conditions. $^\ast$At least 5 control points per side are needed for 1 quartic NURBS element.}
\begin{tabular}{clcccc}
\hline
Method & Number of & \multicolumn{4}{c}{gradient index, $n$} \\
\cline{3-6}
& Control Points & 0 & 0.5 & 1 & 2 \\
\hline
\multirow{8}{*}{SSSS} & IGA-Quadratic & 0.1717 & 0.2324 & 0.2719 & 0.3115 \\
& IGA-Cubic & 0.1717 & 0.2324 & 0.2719 & 0.3115 \\
& IGA-Quartic & 0.1717 & 0.2324 & 0.2719 & 0.3115 \\
& NS-DSG3~\cite{nguyen-xuantran2012} & 0.1721 & 0.2326 & 0.2716 & 0.3107 \\
& ES-DSG3~\cite{nguyen-xuantran2012} & 0.1700 & 0.2296 & 0.2680 & 0.3066 \\
& MITC4~\cite{nguyen-xuantran2012} & 0.1715 & 0.2317 & 0.2704 & 0.3093 \\
& $kp-$Ritz~\cite{leezhao2009} & 0.1722 & 0.2403 & 0.2811 & 0.3221 \\
& MLPG~\cite{gilhooleybatra2007} & 0.1671 & 0.2505 & 0.2905 & 0.3280 \\
\cline{2-6}
\multirow{8}{*}{CCCC} & IGA-Quadratic & 0.0760 & 0.1013 & 0.1183 & 0.1369 \\
& IGA-Cubic & 0.0760 & 0.1014 & 0.1183 & 0.1369 \\
& IGA-Quartic & 0.0760 & 0.1014 & 0.1183 & 0.1369 \\
& NS-DSG3~\cite{nguyen-xuantran2012} & 0.0788 & 0.1051 & 0.1227 & 0.1420 \\
& ES-DSG3~\cite{nguyen-xuantran2012} & 0.0761 & 0.1013 & 0.1183 & 0.1370 \\
& MITC4~\cite{nguyen-xuantran2012} & 0.0758 & 0.1010 & 0.1179 & 0.1365 \\
& $kp-$Ritz~\cite{leezhao2009} & 0.0774 & 0.1034 & 0.1207 & 0.1404 \\
& MLPG~\cite{gilhooleybatra2007} & 0.0731 & 0.1073 & 0.1253 & 0.1444 \\
\hline
\end{tabular}%
\label{tab:ssss-cccc-valid}%
\end{table}%

Next, we illustrate the performance of the present isogeometric method for thin plate problems. A simply supported and a clamped Al/ZrO$_2$-1 square plates subjected to uniform load are considered, while the length-to-thickness ($a/h$) varies from 5 to 10$^6$ and the gradient index ranges from 0 to 2. Two individual approaches are employed: one applied the stabilization technique to eliminate shear locking named S-IGA and the other one, normal IGA, without considering any specific technique for shear locking. The plate is modelled using quadratic NURBS elements with 13$\times$13 control points. The normalized center deflection $\overline{w}_c = 100 w_c \frac{E_c h^3}{12(1-\nu^2)pa^4}$ and the normalized axial stress $\overline{\sigma}_{xx} = \sigma_{xx} \frac{h^2}{p a^2}$ at the top surface of the center of the plate for SSSS and CCCC boundary conditions are depicted in \frefs{fig:SSS_defl_stres} - \ref{fig:CCCC_defl_stres}, respectively. It is observed that IGA results are subjected to shear locking when the plate becomes thin ( $a/h>$ 100). However, the S-IGA results are almost independent of the length-to-thickness ratio for thin plates. The same observations also reported in~\cite{thainguyen-xuan2012} for laminated composite plates. The results using the S-IGA agree very well with those given in~\cite{nguyen-xuantran2012} using the NS-DSG3 element. 

% normalized center deflection and normalized stress...simply supported plate
\begin{figure}[htpb]
\centering
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig1a}}
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig1b}}
\caption{The normalized center deflection, $\overline{w}_c$ and the normalized axial stress $\overline{\sigma}_{xx}$ as a function of $a/h$ for a simply supported Al/Zr0$_2$-1 FGM square plate subjected to a uniform load, $p$: (a) normalized center deflection and (b) normalized center stress.}
\label{fig:SSS_defl_stres}
\end{figure}

% normalized center deflection and normalized stress...clamped plate
\begin{figure}[htpb]
\centering
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig2a}}
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig2b}}
\caption{The normalized center deflection, $\overline{w}_c$ and the normalized axial stress $\overline{\sigma}_{xx}$ as a function of $a/h$ for a clamped Al/Zr0$_2$-1 FGM square plate subjected to a uniform load, $p$: (a) normalized center deflection and (b) normalized center stress.}
\label{fig:CCCC_defl_stres}
\end{figure}

\subsection*{FGM plates under thermo-mechanical loads}
Here, the present isogeometric method is verified on FGM plates subjected to thermo-mechanical loads. A simply supported Al/ZrO$_2$ plate with aluminium at the bottom surface and zirconia at the top surface is considered. The plate with length $a=$ 0.2 m and thickness h=0.01 m is modelled employing quadratic NURBS elements. For comparison, a mesh with 13 control points per side is used. At first, we study the behaviour of SSSS Al/ZrO$_2$-I FGM plate under a uniform mechanical load. \fref{fig:SS_centerline_stres_fgm1} shows the distributions of the normalized axial stress through the thickness of the plate computed for different values of the gradient index $n$. The results are in excellent agreement with those given in~\cite{gilhooleybatra2007,nguyen-xuantran2012}. \fref{fig:SS_centerline_stres_fgm2} plots the central deflection $\overline{w}_c = 100 w_c \frac{E_c h^3}{12(1-\nu^2)pa^4}$ of the plate with respect to various load parameters, $\overline{p} = pa^4/(E_mh^4)$, given in the interval [-14, 0] for different values of the gradient index $n$. It can be seen that the central deflection of the plate linearly increases with respect to the load. It is also observed that the central deflection increases with the gradient index $k$. As expected, the metallic plate has the largest deflection, while the ceramic plate has the lowest. Note that the results match well with those given in~\cite{nguyen-xuantran2012,crocevenini2007}. \fref{fig:SS_centerline_stres_fgm2} shows the normalized axial stress at points on the vertical line passing through the centroid of simply supported Al/ZrO$_2$-2 FGM square plate subjected to a uniform mechanical load $p$. The results agree well with the results reported in~\cite{leezhao2009,nguyen-xuantran2012}. It is observed that for isotropic plates $(i.e, n = 0)$ the axial stress distribution is linear while it is nonlinear for FGM plates. For FGM plates, the magnitude of the axial stress at the bottom is less than the one at the top. The maximum compressive stress at the top surface of the plate has been obtained for the FGM plate with $n=$ 2, whilst the metallic only or ceramic only plates has the minimum tensile stress at the bottom surface.

% normalized stress at points on the vertical line passing through the centroid of SS FGM - 1 square
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/fig3}
\caption{The normalized axial stress $\overline{\sigma}_{xx} = \sigma_{xx} \frac{h^2}{p L^2}$ at points on the vertical line passing through the centroid of a simply supported square Al/Zr0$_2$ FGM plate subjected to uniform mechanical load $p$. }
\label{fig:SS_centerline_stres_fgm1}
\end{figure}

% normalized stress at points on the vertical line passing through the centroid of SS FGM - 1 square
\begin{figure}[htpb]
\centering
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig4}}
\subfigure[]{\includegraphics[scale=0.5]{./Figures/fig5}}
\caption{The normalized center deflection $\overline{w}_c$ and the normalized axial stress $\overline{\sigma}_{xx}$ of a simply supported square Al/Zr0$_2$ FGM plate subjected to uniform mechanical load $p$: (a)The normalized center deflection, $\overline{w}_c = w_c/h$with $\overline{p} = pa^4/(E_mh^4)$ and (b) The normalized axial stress $\overline{\sigma}_{xx} = \sigma_{xx} \frac{h^2}{p a^2}$ at points on the vertical line passing through the centroid with load $p$. }
\label{fig:SS_centerline_stres_fgm2}
\end{figure}

% thermal loads
\subsection*{FGM plates subjected to thermal loading}
Next, we study the behaviour of FGM plates under the thermal loading. A Al/ZrO$_2$-2 FGM plate with length $a=$ 0.2m and thickness $h=$ 0.01m is considered. The temperature at the top surface of the plate is varied from 0$^\circ$C to 500$^\circ$C, while the temperature at the bottom surface is maintained at 20$^\circ$C. The temperature of the stress free state is assumed to be at $T_o=$ 0$^\circ$C. \fref{fig:SS_normDisp_thermal} depicts the non-dimensional center deflection of the plate under the thermal load. This problem was solved by Zhao and Liew, using the element free $kp$-Ritz method~\cite{zhaoliew2009} and by Xuan \textit{et al.,}~\cite{nguyen-xuantran2012} using NS-DSG3 elements. The results obtained with our IGA method agree very well with those given in~\cite{zhaoliew2009,nguyen-xuantran2012}. From \fref{fig:SS_normDisp_thermal}, it is observed that the metal plate gives the maximum deflection because of its high thermal conductivity. The deflection of the FGM plate with the gradient index $n=1$ is minimum. Generally, it can be seen that the deflections of the FGM plates are much lower than those of isotropic plates $(i.e., n = 0)$, which implies high temperature resistance behaviour of the functionally graded plates.

% normalized center deflection of SS FGM - 2 square
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/fig10}
\caption{The normalized center deflection $\overline{w}_c = w_c/h$ of a simply supported square Al/ZrO$_2$ FGM plate subjected to thermal load. }
\label{fig:SS_normDisp_thermal}
\end{figure}

Now, we investigate the FGM plate under thermo-mechanical loads. The temperature at the top surface of the plate is held at 300$^\circ$C (top surface is assumed to be rich in ceramic) and the temperature at the bottom surface (assumed to be rich in metal) is $T_m=$20$^\circ$C. \fref{fig:SS_normDisp_thermoMech_fgm2} shows the center deflection $\overline{w}_c = w_c/h$ of the plate with respect to various load parameters $\overline{p} = pa^4/(E_mh^4)$ given in the interval -14 $\le \overline{p} \le$ 0 for different values of the gradient index. It can be seen that the central deflection of the plate is completely different from the case with a purely mechanical loading  (see \fref{fig:SS_centerline_stres_fgm2}). However, similarly to the case of the FGM plate under pure mechanical loading, the center deflection of the plate linearly increases with the load. The metallic phase shows the maximum range of deflection changes and  the ceramic plate the least.

% normalized center deflection of FGM-2 with thermal load
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/fig11}
\caption{The normalized center deflection $\overline{w}_c = w_c/h$ of a simply supported square Al/ZrO$_2$ FGM plate subjected to thermo-mechanical load. }
\label{fig:SS_normDisp_thermal_fgm2}
\end{figure}

% normalized center deflection of FGM-2 with thermal load
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/fig12}
\caption{The normalized center deflection $\overline{w}_c = w_c/h$ of a simply supported square Al/ZrO$_2$ FGM plate subjected to thermo-mechanical load. }
\label{fig:SS_normDisp_thermoMech_fgm2}
\end{figure}

\fref{fig:SS_normDisp_thermoMech_fgm2} plots the distribution of axial stress through the thickness of the plate under the uniform mechanical load $p=$ -10$^6$ N/m$^2$. Comparing to \fref{fig:SS_centerline_stres_fgm2} for purely mechanical load, it is seen that the maximum compressive stress at the top surface of the plate has been obtained for the FGM plate with a gradient index $n=$ 1. Again, the metallic or ceramic plate shows the minimum tensile stress at the bottom surface. Note that the results match very well with those given in~\cite{zhaoliew2009,nguyen-xuantran2012}.

%------------------------------------------------------
\subsection*{Skew plates}
In this example, we study the behaviour of FGM skew plates under mechanical loads. A simply supported Al/ZrO$_2$ FGM skew plate with length $a=$ 10m and thickness $h=$ 0.1m is considered. The plate is subjected to a uniform mechanical load $p=$ -10$^4$ N/m$^2$. A mesh of quadratic NURBS elements with 17 $\times$ 17 control points is used for modelling the plate. \fref{fig:skewMechLoadn05} shows the distribution of non-dimensional axial stress $\overline{\sigma}_{xx} = \sigma_{xx} h^2/(pa^2)$ through the thickness of the plate for different skew angles with gradient index $n=$ 0.5. It can be observed that the axial stresses increase as the skew angle decreases. Similar behaviour can be found for gradient indices $n=$ 1 and $n=$ 2 in \frefs{fig:skewMechLoadn1} and \ref{fig:skewMechLoadn2}, respectively. The results obtained by our isogeometric analysis are in a good agreement with those reported in \cite{leezhao2009} using the element free $kp-$ Ritz method and the results of NS-DSG3~\cite{nguyen-xuantran2012} and ES-DSG3~\cite{nguyen-xuantran2011}.

% effect of skew angle on the axial stress...n = 0.5
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/fig13}
\caption{The effect of skew angle on the axial stress $\overline{\sigma}_{xx} = \sigma_{xx} \frac{h^2}{pL^2}$ profile for simply supported FGM Al/ZrO$_2$ subjected to a mechanical load with gradient index $n=$ 0.5.}
\label{fig:skewMechLoadn05}
\end{figure}

% effect of skew angle on the axial stress...n = 1
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/fig14}
\caption{The effect of skew angle on the axial stress $\overline{\sigma}_{xx} = \sigma_{xx} \frac{h^2}{pL^2}$ profile for simply supported FGM Al/ZrO$_2$ subjected to a mechanical load with gradient index $n=$ 1.0.}
\label{fig:skewMechLoadn1}
\end{figure}

% effect of skew angle on the axial stress...n = 2
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.5]{./Figures/fig15}
\caption{The effect of skew angle on the axial stress $\overline{\sigma}_{xx} = \sigma_{xx} \frac{h^2}{pL^2}$ profile for simply supported FGM Al/ZrO$_2$ subjected to a mechanical load with gradient index $n=$ 2.0.}
\label{fig:skewMechLoadn2}
\end{figure}
